Do Performance Aspirations Matter for Guiding Software Configuration Tuning?

Configurable software systems can be tuned for better performance. Leveraging on some Pareto optimizers, recent work has shifted from tuning for a single, time-related performance objective to two intrinsically different objectives that assess distinct performance aspects of the system, each with varying aspirations. Before we design better optimizers, a crucial engineering decision to make therein is how to handle the performance requirements with clear aspirations in the tuning process. For this, the community takes two alternative optimization models: either quantifying and incorporating the aspirations into the search objectives that guide the tuning, or not considering the aspirations during the search but purely using them in the later decision-making process only. However, despite being a crucial decision that determines how an optimizer can be designed and tailored, there is a rather limited understanding of which optimization model should be chosen under what particular circumstance, and why. In this paper, we seek to close this gap. Firstly, we do that through a review of over 426 papers in the literature and 14 real-world requirements datasets. Drawing on these, we then conduct a comprehensive empirical study that covers 15 combinations of the state-of-the-art performance requirement patterns, four types of aspiration space, three Pareto optimizers, and eight real-world systems/environments, leading to 1,296 cases of investigation. We found that (1) the realism of aspirations is the key factor that determines whether they should be used to guide the tuning; (2) the given patterns and the position of the realistic aspirations in the objective landscape are less important for the choice, but they do matter to the extents of improvement; (3) the available tuning budget can also influence the choice for unrealistic aspirations but it is insignificant under realistic ones.

==> tables/count1.tex <==
\begin{table}[t!]
\caption{Total count of wins and $\hat{A}_{12}$ levels over 1080 cases.}
\label{tb:rel-count}
%\setlength{\tabcolsep}{1.1mm}
\footnotesize
\centering
\begin{tabular}{lcccc}\toprule

&\textbf{L}&\textbf{M}&\textbf{S}&\textbf{Total Wins (non-trivial $\hat{A}_{12}$)}\\
\midrule


\texttt{PS-w}&454&66&24&657 (544)\\
\texttt{PS-w/o}&90&17&20&175 (127)\\

\bottomrule
\end{tabular}
\centering
 \begin{tablenotes}
    \footnotesize
    \item L, M, and S denotes large, medium, and small $\hat{A}_{12}$, respectively. For all non-trivial $\hat{A}_{12}$ cases, only those with $p<0.05$ are considered.
    \end{tablenotes}
\end{table}

==> tables/count2.tex <==
\begin{table}[t!]
\caption{Total count of wins and $\hat{A}_{12}$ levels over 216 cases.}
\label{tb:unr-count}
%\setlength{\tabcolsep}{1.1mm}
\footnotesize
\centering
\begin{tabular}{lcccc}\toprule

&\textbf{L}&\textbf{M}&\textbf{S} &\textbf{Total Wins (non-trivial $\hat{A}_{12}$)}\\
\midrule


\texttt{PS-w}&25&10&6&65 (41)\\
\texttt{PS-w/o}&83&28&18&139 (129)\\

\bottomrule
\end{tabular}
\centering
  \begin{tablenotes}
    \footnotesize
    \item L, M, and S denotes large, medium, and small $\hat{A}_{12}$, respectively. For all non-trivial $\hat{A}_{12}$ cases, only those with $p<0.05$ are considered.
    \end{tablenotes}
\end{table}

==> tables/rq3-t1.tex <==
\begin{table}
\caption{Best combinations of patterns ($\mathbfcal{P}'$) that guide \texttt{PS-w} under each realistic requirement ($\mathbfcal{P}$) over all cases.}
\label{tb:rq3-t1}
%\setlength{\tabcolsep}{1mm}
\centering
\footnotesize
\begin{tabular}{ll}\toprule


\textbf{Requirements} ($\mathbfcal{P}$)&\textbf{Combination of Patterns} ($\mathbfcal{P}'$)\\

\midrule

$\{\vect{p_0}\textit{,}\vect{p_1}\}$&$\{\vect{p_0}\textit{,}\vect{p_1}\}$, $\{\vect{p_3}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_1}\textit{,}\vect{p_0}\}$&$\{\vect{p_2}\textit{,}\vect{p_0}\}$\\

$\{\vect{p_0}\textit{,}\vect{p_2}\}$&$\{\vect{p_0}\textit{,}\vect{p_1}\}$, $\{\vect{p_3}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_2}\textit{,}\vect{p_0}\}$&$\{\vect{p_2}\textit{,}\vect{p_0}\}$\\

$\{\vect{p_0}\textit{,}\vect{p_3}\}$&$\{\vect{p_3}\textit{,}\vect{p_3}\}$\\

$\{\vect{p_3}\textit{,}\vect{p_0}\}$&$\{\vect{p_3}\textit{,}\vect{p_0}\}$\\

$\{\vect{p_1}\textit{,}\vect{p_1}\}$&$\{\vect{p_0}\textit{,}\vect{p_2}\}$, $\{\vect{p_3}\textit{,}\vect{p_0}\}$, $\{\vect{p_3}\textit{,}\vect{p_2}\}$\\

$\{\vect{p_2}\textit{,}\vect{p_2}\}$&$\{\vect{p_0}\textit{,}\vect{p_2}\}$, $\{\vect{p_3}\textit{,}\vect{p_2}\}$\\

$\{\vect{p_3}\textit{,}\vect{p_3}\}$&$\{\vect{p_3}\textit{,}\vect{p_3}\}$\\

$\{\vect{p_1}\textit{,}\vect{p_2}\}$&$\{\vect{p_0}\textit{,}\vect{p_2}\}$, $\{\vect{p_3}\textit{,}\vect{p_2}\}$\\

$\{\vect{p_2}\textit{,}\vect{p_1}\}$&$\{\vect{p_0}\textit{,}\vect{p_2}\}$, $\{\vect{p_3}\textit{,}\vect{p_0}\}$, $\{\vect{p_3}\textit{,}\vect{p_2}\}$\\


$\{\vect{p_1}\textit{,}\vect{p_3}\}$&$\{\vect{p_2}\textit{,}\vect{p_0}\}$\\





$\{\vect{p_3}\textit{,}\vect{p_1}\}$&$\{\vect{p_3}\textit{,}\vect{p_1}\}$, $\{\vect{p_0}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_2}\textit{,}\vect{p_3}\}$&$\{\vect{p_2}\textit{,}\vect{p_0}\}$\\

$\{\vect{p_3}\textit{,}\vect{p_2}\}$&$\{\vect{p_0}\textit{,}\vect{p_2}\}$, $\{\vect{p_0}\textit{,}\vect{p_1}\}$, $\{\vect{p_3}\textit{,}\vect{p_2}\}$\\







\bottomrule
\end{tabular}
\end{table}

==> tables/rq3-t2.tex <==
\begin{table}
\caption{Best combinations of patterns ($\mathbfcal{P}'$) that guide \texttt{PS-w} under each unrealistic requirement ($\mathbfcal{P}$) over all cases.}
\label{tb:rq3-t2}
%\setlength{\tabcolsep}{1mm}
\centering
\footnotesize
\begin{tabular}{ll}\toprule


\textbf{Requirements} ($\mathbfcal{P}$)&\textbf{Combination of Patterns} ($\mathbfcal{P}'$)\\

\midrule

$\{\vect{p_1}\textit{,}\vect{p_1}\}$&$\{\vect{p_1}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_2}\textit{,}\vect{p_2}\}$&$\{\vect{p_1}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_3}\textit{,}\vect{p_3}\}$&$\{\vect{p_1}\textit{,}\vect{p_1}\}$, $\{\vect{p_2}\textit{,}\vect{p_1}\}$, $\{\vect{p_3}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_1}\textit{,}\vect{p_2}\}$&$\{\vect{p_1}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_2}\textit{,}\vect{p_1}\}$&$\{\vect{p_1}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_1}\textit{,}\vect{p_3}\}$&$\{\vect{p_1}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_3}\textit{,}\vect{p_1}\}$&$\{\vect{p_1}\textit{,}\vect{p_1}\}$, $\{\vect{p_3}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_2}\textit{,}\vect{p_3}\}$&$\{\vect{p_1}\textit{,}\vect{p_1}\}$\\

$\{\vect{p_3}\textit{,}\vect{p_2}\}$&$\{\vect{p_2}\textit{,}\vect{p_1}\}$, $\{\vect{p_3}\textit{,}\vect{p_1}\}$\\







\bottomrule
\end{tabular}
\end{table}
